SAL-PIM: A Subarray-level Processing-in-Memory Architecture with LUT-based Linear Interpolation for Transformer-based Text Generation

Text generation is a compelling sub-field of natural language processing, aiming to generate human-readable text from input words. In particular, the decoder-only generative models, such as generative pre-trained transformer (GPT), are widely used for text generation, with two major computational stages: summarization and generation. Unlike the summarization stage, which can process the input tokens in parallel, the generation stage is difficult to accelerate due to its sequential generation of output tokens through iteration. Moreover, each iteration requires reading a whole model with little data reuse opportunity. Therefore, the workload of transformer-based text generation is severely memory-bound, making the external memory bandwidth system bottleneck. In this paper, we proposed a subarray-level processing-in-memory architecture named SAL-PIM, HBM-based PIM architecture for the end-to-end acceleration of transformer-based text generation. The SAL-PIM architecture includes three architectural features. First, the SAL-PIM architecture utilizes higher internal bandwidth by integrating multiple subarray-level arithmetic logic units with optimized data mapping schemes. Second, the SAL-PIM architecture adopts LUT-based linear interpolation to perform complex non-linear functions in PIM. Third, the SAL-PIM architecture accelerates end-to-end inference on PIM in text generation. Furthermore, to validate the SAL-PIM architecture, we built cycle-accurate simulator and implemented the SAL-PIM's logic units in 28-nm CMOS technology. As a result, when the input size is from 32 to 128 and the output size is from 1 to 256, SAL-PIM achieves a maximum of 4.72 times speedup and an average of 1.83 times speedup for the text generation based on the GPT-2 medium model compared to the server-level GPU.

==> 11_review.tex <==
\onecolumn
\renewcommand{\thefigure}{A\arabic{figure}}

\setcounter{figure}{0}

\section{Responses to Reviewers}

\textbf{For all the reviewers}

We thank all the reviewers for insightful and constructive comments. We believe the revision based on your valuable comments has improved the quality of our paper, and any revisions are marked with red for your convenience. The following list summarizes the changes of the tables and figures in the revised manuscript.
\newline 

\textcolor{red}{\textbf{- Table \ref{table_Review} is added in Section \ref{sec:background}.2 on Page 4.}}
\newline  

\textcolor{red}{\textbf{- Table \ref{table_1} (previously Table 1) is revised in Section \ref{sec:evaluation}.1 on Page 9.}}
\newline  

\textcolor{red}{\textbf{- Figure \ref{fig_11} is revised in Section \ref{sec:evaluation}.3 on Page 10.}}
\newline  

\textcolor{red}{\textbf{- Figure \ref{fig_review} is added in Section \ref{sec:detailed_analysis}.2 on Page 11.}}
\newline  


\textbf{Reviewer: 1}

The motivation for the paper is strong and presented well. I enjoyed reading the paper as and found the overall and I found the techniques and mechanisms described sensible overall. What I found disappointing is the analysis and discussion of results and also of related work. Some specifics below:
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 1-1
1. The maximum speedup seems larger than the BW advantage -- how and why? 
\newline

\textcolor{blue}{\textbf{Response}: We appreciate the reviewer for bringing this to our attention. Generally, the GPU cannot fully utilize memory bandwidth because it is designed to target general tasks that require higher computational parallelism. The GPU exhibits high utilization in certain operations like GEMM, while others may not achieve the same utilization level. However, the SAL-PIM architecture aims to accelerate transformer-based text generation through optimized mapping schemes and dataflows. Consequently, achieving a higher speedup than the benefits of memory bandwidth is possible. We included additional explanations regarding the performance gain in Section \ref{sec:evaluation}.3 in the revised manuscript. The following paragraph has been added as new content.}
\newline 

\textcolor{red}{\textbf{Section \ref{sec:evaluation}.3 on Page 10}: "This result indicates the maximum speedup greater than the gain obtained from subarray-level parallelism. It is because GPUs are designed to support general tasks and typically do not fully utilize the memory bandwidth. In contrast, SAL-PIM enables optimized operations due to its use of optimized data mapping and dataflow targeted to accelerate transformer-decoder-based text generation."}
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 1-2
2. The area analysis seems way off. You are citing a paper from 1999! You are also substantially changing the bank design and it does not seem reasonable to just add the area overhead estimated for the units -- the whole layout is changing and how is not really discussed. Furthermore the costs seem quite different than those of recent prototypes that are cited in the paper. Why, how come, ... ? 
\newline

\textcolor{blue}{\textbf{Response}: We thank the reviewer for pointing this out. Although the paper was written in 1999 and can be considered relatively old, it is still regarded as reliable in the field. Numerous state-of-the-art studies(DRISA\cite{li2017drisa}, Fulcrum\cite{lenjani2020fulcrum}, and TransPIM\cite{zhou2022transpim}) have referenced and utilized the scaling methodology described in the paper. We understood your concerns and included the papers as a reference in the revised manuscript. Additionally, regarding the SAL-PIM architecture, the memory cell structure remains relatively the same by simply connecting the S-ALU to the separated GBLs using switches. As a result, the dominant factor contributing to area overhead is the units themselves, while the transistor size for the switch is negligibly small.}
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 1-3
3. You do some comparisons to alternatives, but how about alternatives that are more in line with current prototypes -- i.e., not end to end within DRAM? Seems particularly relevant and appropriate to include such comparisons.
\newline

\textcolor{blue}{\textbf{Response}: We thank the reviewer's suggestion and agree that more evaluation results make our manuscript better. One of the key features of SAL-PIM is the ability to perform end-to-end computations within HBM-PIM, enabling the simulator to measure the inference latency of the entire model. Considering this capability, we believed that it was reasonable to compare SAL-PIM with the actual GPU. While we value the reviewer's advice, the current proposed PIM architectures (FIM\cite{kwon202125} and AiM\cite{lee20221aim}) are practically challenging to execute end-to-end text generation due to their behavior and reliance on the host processor, which makes reliable comparisons difficult. Therefore, we compared and presented speedup for the GEMV operation, which yields the most significant performance gain using the existing PIM architectures.}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 1-4
4. What would happen with larger models? You allude to the longer vectors of GPT-3, but it also has 2 - 3 orders of magnitude more parameters. How would those fit in DRAM? Really, they would not so what would be the impact of communication and the challenges with concatenation?
\newline

\textcolor{blue}{\textbf{Response}: We thank the reviewer for pointing this out. We agree with the need to address memory capacity limitation for the practical implementation of PIM on Large Language Models (LLMs). We anticipate that aggressive pruning, quantization techniques, and the development of efficient interconnection methods will play crucial roles in overcoming these obstacles. Further research and efforts in these areas are warranted. In addition, the larger size model requires a large memory bandwidth. The subarray-level PIM has significant potential to address this issue.} 
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 1-5
5. You assume a frequency speedup for the logic, but it is not clear that it will be possible. If it is, are there are and power implications?
\newline

\textcolor{blue}{\textbf{Response}: We thank the reviewer for pointing this out. Several recent studies, SpAtten\cite{wang2021spatten}, and ELSA\cite{ham2021elsa}, have utilized MAC units operating at a frequency of 1GHz in logic technology. In recent PIM research (H. Shin et al., 2018), it was mentioned that despite the possibility of implementing MAC units at 1GHz, a MAC unit operating at a lower frequency was designed due to time constraints of DRAM. Moreover, when we implemented the MAC units using a standard cell library and the MAC units were sufficient to operate at a frequency higher than 800MHz. Considering that the performance degradation between DRAM and logic technology is 22\%, and the peripheral circuit on real DRAM operates at 1GHz, the MAC unit operated at 500MHz is possible. The higher operating frequency causes the increasing power consumption, and the increment was considered in table \ref{table_2}. We added the explanation about area overhead in Section \ref{sec:circuit}.1 in the revised manuscript. The following paragraph has been added as new content.}
\newline

\textcolor{blue}{H. Shin, D. Kim, E. Park, S. Park, Y. Park and S. Yoo, "McDRAM: Low Latency and Energy-Efficient Matrix Computations in DRAM," in IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems, vol. 37, no. 11, pp. 2613-2622, Nov. 2018, doi: 10.1109/TCAD.2018.2857044.}
\newline

\textcolor{red}{\textbf{Section \ref{sec:circuit}.1 in Page 7}: "Several recent studies, including \cite{wang2021spatten, ham2021elsa}, have utilized MAC units operating at a frequency of 1GHz in logic technology. On the other hands, ALUs in recent PIM works can be only utilized at 250MHz.", "We implemented shared MAC using a standard cell library to verify its feasibility, achieving a clock frequency of over 800MHz. Considering the 22\% performance degradation between DRAM and logic technology, it is confirmed that the shared MACs are feasible."}
\newline 

\newpage

\textbf{Reviewer: 2}

- The paper flow is good, all writing and diagrams are clear and understandable. The work is novel, being the first to accelerate a GPT based workload end-end in DRAM based PIM.

- Interpolation through linear fitting to compute non-linear functions is novel and its evaluation shows promising results.

- The near memory architecture to perform MACs is straightforward (LBLs -- GBLs), although the design choice to include the number of compute units (trading off throughput for area) and the circuit design of S-ALU and C-ALU is novel.

- The design is modular, allocating different functions to similar hardware by breaking down different functions to similar calculations.

- The evaluation is detailed but comparison with other works is not, i.e., the comparison in Fig. 12 and Fig. 11 can be done using TOPs and TOPs/w instead of calculated speedup.
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 2-1
1. Due to the application’s complex nature, the reader is completely lost on how the data flow occurs in the circuit/architecture. The overall compute is broken down to General Matrix multiplications, non-linear function interpolation and multi-head operations. Section 3 briefs on the mapping of these operations alone and does not provide a full algorithmic mapping as this work claims to accelerate all compute in Fig. 2. Section 3 can be rewritten to explain the data flow instead of data mapping and interleave the data mapping and specific compute explanation in section 4.
\newline

\textcolor{blue}{\textbf{Response}: Thanks for the suggestion. 
We agree that explaining the dataflow is helpful for readers' understanding. However, we believe that the contents of Section \ref{sec:architecture}.2.1 are necessary to explain the importance of mapping in GPT. Therefore, we added explanation about dataflow for GPT in SAL-PIM in Section \ref{sec:architecture}.2.1.}
\newline

\textcolor{red}{\textbf{Section \ref{sec:architecture}.2.1 is added.}}
\newline 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 2-2
2. In the S-ALU architecture, the mem read and write is said to be slower than the digital compute of MACs, so the architecture uses half the number of adders/multipliers at 500Mhz instead of using the same number of Adders at a lower frequency, i.e., pipelining. Further circuit level improvements (area and throughput) could’ve been made by using gather scatter modules and pipeline deeper for the MAC calculations.
\newline

\textcolor{blue}{\textbf{Response}: Thanks for the insightful suggestion. The real speed of the DRAM core is limited(250MHz), and implementing complicated modules at the subarray-level causes a larger area overhead. Therefore, we decided to include only the minimum necessary units at the subarray-level, and we have not utilized pipelining at the 500MHz frequency. To verify operation without pipelining, we implemented the MAC units using the standard cell library, achieving operation up to 800MHz. Even considering a 22\% performance degradation due to the DRAM technology, operation at 500MHz is still feasible. Although pipelining may be less necessary in the SAL-PIM architecture, we believe that employing pipelining for the in-memory ALU can increase throughput and create various opportunities.}
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 2-3
3. Some important hardware level information is lacking regarding the cycles of operation, raw throughput of each the designed component e.g., S-ALU, C-ALU etc., and performance estimation (Latency and power) starting from read-outs of DRAM to the final generated output and how that output evaluates to in the algorithm.
\newline

\textcolor{blue}{\textbf{Response}: We appreciate the reviewer for bringing this to our attention. The operation of S-ALU and C-ALU is synchronized with the read operation of SAL-PIM, resulting in the same latency. Therefore, S-ALUs and C-ALUs are expected to achieve the same throughput as the bandwidth available at subarrays and channels in SAL-PIM, respectively. We acknowledge the need for additional explanations regarding the power starting from the read-out of DRAM in our paper. We agree that the measurements for power consumption would enhance the reader's understanding. Therefore, we added the graph and some explanation in the revised manuscript.}
\newline

\textcolor{red}{\textbf{Figure \ref{fig_review} is added.}}
\newline

\textcolor{red}{\textbf{Section \ref{sec:detailed_analysis}.2 on Page 11}: "Subarray-level parallelism offers increased bandwidth but consumes more energy. Operating multiple banks and subarrays simultaneously result in higher energy consumption compared to conventional DRAM operations. However, it provides advantages for energy due to the shorter data movement distances. Figure \ref{fig_review} illustrates the power consumption of SAL-PIM for various values of $P_{Sub}$."}

\textcolor{red}{\textbf{Section \ref{sec:detailed_analysis}.2 on Page 11}: "In our evaluation, we conducted 32 token generations using the GPT-2 medium model. The energy consumption was assigned as follows\cite{o2017fine}: $e_{act}=909pJ$, $e_{pre-gsa}=1.51pJ/bit$, $e_{post-gsa}=1.17pJ/bit$, and $e_{io}=0.80pJ/bit$. We assumed that 26\% of the total HBM poewr budget is allocated for refresh operations\cite{shin2017extreme}. As depicted in Figure \ref{fig_review}, when $P_{Sub}$ is 1 or 2, the power consumption remains significantly lower than the power budget, while for $P_{Sub}$ is 4, it exceeds the power budget by 15.5\%. Despite this, considering the high power usage expected for computations in CPUs or GPUs, SAL-PIM can still be considered sufficiently power-efficient for transformer-decoder-based text generation."}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 2-4
4. More accuracy vs no of sections for interpolation will bolster the design choice of using 32 sections.
\newline

\textcolor{blue}{\textbf{Response}: We thank the reviewer for pointing this out. As mentioned in Section 2.3, there is no accuracy loss when the number of sections exceeds 32. However, we chose for 64 sections for linear interpolation due to two reasons. Firstly, we included a margin to accommodate other model adaptations. Secondly, when 32 sections are chosen, they all fit within a single row. By selecting 64 sections, we aimed to demonstrate the scalability in the subarray direction of the SAL-PIM architecture. It's important to note that while the accuracy remains unaffected, this configuration allowed us to showcase the flexibility and scalability of our approach.}
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 2-5
5. The authors draw comparison with only one other PIM based solution, more detailed comparison is required with power numbers and throughput in terms of operations. No reason is provided on why only [13] was picked to compare bank level MACs/GEMV and why other works are neglected.
\newline

\textcolor{blue}{\textbf{Response}: Thanks for pointing this out. The main goal of SAL-PIM is accelerating end-to-end text generation, and we conducted a performance evaluation by comparing it with GPU. Comparing SAL-PIM architecture with bank-level PIM alone would not be appropriate since bank-level PIM is mainly limited to accelerating GEMV operations and can only perform part of the end-to-end process. In our comparison with the bank-level PIM, we intended to assess whether the higher bandwidth available in our approach could be effectively utilized for GEMV operations, which are the most profitable in PIM. The results demonstrated a significant speedup of nearly four times. Hence, we specifically compared our approach with Newton\cite{he2020newton}, which is a well-known representative of bank-level PIM. Similar comparisons with other bank-level PIM implementations would yield similar results. We included explanations in Section \ref{sec:evaluation}.4 in the revised manuscript. The following paragraph has been added as new content.}
\newline 

\textcolor{red}{\textbf{Section \ref{sec:evaluation}.4 on Page 10}: "SAL-PIM architecture has a much higher maximum bandwidth compared to Bank-level PIM, so we evaluated the SAL-PIM architecture compared to the bank-level PIM architecture to verify whether this high bandwidth is being fully utilized is necessary."}
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 2-6
6. Section 7.1 and 7.2 will be more meaningful if they are demonstrated as comparison tables rather than text.
\newline

\textcolor{blue}{\textbf{Response}: Thanks for the suggestion. In our paper, we primarily discussed relevant PIM studies in Section \ref{sec:introduction} (Introduction) and Section \ref{sec:background} (Background). In Section \ref{sec:related} (Related Works), we referred to previous studies, including non-PIM accelerators and PIMs with look-up tables. We agree that including the table would be more helpful, and we added the table in Section \ref{sec:background}.2.}
\newline

\textcolor{red}{\textbf{Table \ref{table_Review} is added on Page 4.}}
\newline

\textcolor{red}{\textbf{Section \ref{sec:background}.2 on Page 4}: "Table \ref{table_Review} summarizes DRAM-based PIMs"}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Reviewer: 3}

Given the large work on near-DRAM-bank ALUs, the contributions of this paper are incremental. The key innovation is the use of LUTs as a way to reduce the high computational overhead of non-linear functions in language generation models. 
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 3-1
1. While this is the key innovation, the comparisons in the results don't really highlight this aspect. The authors only report a performance comparison (Fig 12) against the baseline Bank-Level PIM - but as the authors show, modifying Psub can impact this performance (Fig 14). What is really needed is a comparison of performance, energy, area for these different design points (different Psub), but Table 2 only reports this for a single design point.
\newline

\textcolor{blue}{\textbf{Response}: Thanks for the suggestion. What we aim to show in Figure \ref{fig_12} is the bandwidth utilization in subarray-level parallelism. Therefore, the best way to demonstrate this is by comparing the results when $P_{Sub}$ is 4. We added an explanation for this in Section \ref{sec:evaluation}.4. Additionally, we considered your suggestion of incorporating various values of $P_{Sub}$ and conducted additional evaluations to update Figure \ref{fig_11} in the revised manuscript. This modification enables us to showcase the performance improvement across multiple $P_{Sub}$ values. Moreover, we have included a graph and its corresponding explanation in Section \ref{sec:detailed_analysis}.2, demonstrating the power consumption for different $P_{Sub}$ values. The following paragraph has been added as new content.}
\newline

\textcolor{red}{\textbf{- Table \ref{table_1} (previously Table 1) is revised in Section \ref{sec:evaluation}.1 on Page 9.}}
\newline  

\textcolor{red}{\textbf{- Figure \ref{fig_11} is revised in Section \ref{sec:evaluation}.3 on Page 10.}}
\newline  

\textcolor{red}{\textbf{- Figure \ref{fig_review} is added in Section \ref{sec:detailed_analysis}.2 on Page 11.}}
\newline  

\textcolor{red}{\textbf{Section \ref{sec:evaluation}.4 on Page 10}: "SAL-PIM architecture has a much higher maximum bandwidth compared to Bank-level PIM, so we evaluated the SAL-PIM architecture compared to the bank-level PIM architecture to verify whether this high bandwidth is being fully utilized is necessary."}
\newline

\textcolor{red}{\textbf{Section \ref{sec:detailed_analysis}.2 on Page 11}: "Subarray-level parallelism offers increased bandwidth but consumes more energy. Operating multiple banks and subarrays simultaneously result in higher energy consumption compared to conventional DRAM operations. However, it provides advantages for energy due to the shorter data movement distances. Figure \ref{fig_review} illustrates the power consumption of SAL-PIM for various values of $P_{Sub}$."}
\newline

\textcolor{red}{\textbf{Section \ref{sec:detailed_analysis}.2 on Page 11}: "In our evaluation, we conducted 32 token generations using the GPT-2 medium model. The energy consumption was assigned as follows: $e_{act}=909pJ$, $e_{pre-gsa}=1.51pJ/bit$, $e_{post-gsa}=1.17pJ/bit$, and $e_{io}=0.80pJ/bit$\cite{o2017fine}. We assumed that 26\% of the total HBM poewr budget is allocated for refresh operations\cite{shin2017extreme}. As depicted in Figure \ref{fig_review}, when $P_{Sub}$ is 1 or 2, the power consumption remains significantly lower than the power budget, while for $P_{Sub}$ is 4, it exceeds the power budget by 15.5\%. Despite this, considering the high power usage expected for computations in CPUs or GPUs, SAL-PIM can still be considered sufficiently power-efficient for transformer-decoder-based text generation."}
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 3-2
2. Another concern is the use of a non-DRAM process for area and energy estimations. The authors use a scaling factor from a 1999 paper [31]; is there a more recent analysis that reports a more appropriate scaling? And PrimePower needs a citation too. The 25\% threshold for acceptable area impact is far too high.
\newline

\textcolor{blue}{\textbf{Response}: We thank the reviewer for pointing this out. Although the paper was written in 1999 and can be considered relatively old, it is still regarded as reliable in the field for scaling area between logic and DRAM technology. Many state-of-the-art studies(DRISA\cite{li2017drisa}, Fulcrum\cite{lenjani2020fulcrum}, and TransPIM\cite{zhou2022transpim}) have referenced and utilized the scaling methodology described in the paper, and we adopt it as well. We added more recent papers to the reference in the revised manuscript.}

\textcolor{blue}{We added the citation of PrimePower in Section \ref{sec:evaluation}.2 in the revised manuscript.}

\textcolor{blue}{The 25\% threshold was mentioned in Newton\cite{he2020newton}, which is researched by a DRAM vendor, so we think the threshold is reliable. In addition, the SAL-PIM architecture has only 2.91\% area overhead, further lower than the threshold.}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 3-3
3. Fig 3 shows that the non-linear functions contribute less than a quarter of total execution time. The improvements reported later are much higher. So if the authors believe that acceleration improves the other phases and the contribution of non-linear layers is higher, they should show that as well. 
\newline

\textcolor{blue}{\textbf{Response}: We thank the reviewer for pointing this out. Figure \ref{fig_3} shows the breakdown of execution time on the GPU. As we mentioned in Section \ref{sec:background}.1, n, if the MHA and FFN are accelerated, the portion of non-linear functions is further increased. Moreover, the speedup observed in the SAL-PIM architecture is not solely due to the acceleration of non-linear functions. There are two additional factors that contribute to the SAL-PIM architecture's superior speedup compared to the GPU. Firstly, the increased bandwidth allows for faster computation of GEMV operations, which serves as the primary reason for the performance improvement over the GPU. Secondly, the optimized data mapping and data flow minimize data movement and maximize resource utilization. As a result, the SAL-PIM architecture demonstrates a speedup of 67.83$\times$ compared to the GPU.}
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Review 3-4
4. In general, I had trouble teasing out the impact of the novel contributions of this paper vs. contributions that are also part of prior work like Bank-level PIM. It would really help to show how ALU computation has been replaced with LUT access and the energy cost of doing a computation with ALU vs with LUT. Without that basic comparison, it is difficult to estimate the impact of this work.
\newline

\textcolor{blue}{\textbf{Response}: Thanks for the suggestion. Without LUT, the non-linear function can be computed using Taylor series expansion, as presented in TransPIM\cite{zhou2022transpim}. The fifth-order Taylor series expansion requires ten vector multiplications and six vector additions. However, with the LUT operation, only one vector multiplication and one vector addition are necessary. The key difference between the SAL-PIM architecture and existing bank-level PIM (AiM\cite{lee20221aim}) lies in the multiple LUT operations. The SAL-PIM architecture performs LUT operations for 16 data during a one time read, whereas bank-level PIM processes one data at a time. A detailed comparison of LUT operations can be found in Section \ref{sec:detailed_analysis}.1. We added the explanation in Section \ref{sec:related}.2 in the revised manuscript. The following paragraph has been added as new content.}
\newline

\textcolor{red}{\textbf{Section \ref{sec:related}.2 on Page 11}: "Therefore, SAL-PIM uses LUT-based linear interpolation to support higher bit precision. AiM\cite{lee20221aim} also utilizes LUT-based linear interpolation to support various activation functions. However, it is limited to supporting activation functions and is only applied to the result data of a bank-level adder tree. On the other hand, SAL-PIM supports a wide range of non-linear functions and utilizes LUT-embedded subarrays to apply LUT-based linear interpolation to multiple data at once."}
\newline 

==> acknowledgment.tex <==
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The authors would like to thank...
